A Hybrid Antenna Switching Scheme for Dynamic Channel Sounding

Channel sounding is essential for the development of radio systems. One flexible strategy is the switched-array-based channel sounding, where antenna elements are activated at different time instants to measure the channel spatial characteristics. Although its hardware complexity is decreased due to fewer radio-frequency (RF) chains, sequentially switching the antenna elements can result in aliasing in the joint estimation of angles and Doppler frequencies of multipath components (MPCs). Therefore, pseudo-random switching has been proposed to mitigate such aliasing and increase estimation accuracy in both angular and Doppler domains. Nevertheless, the increased Doppler resolution could cause additional post-processing complexity of parameter estimation, which is relevant when the Doppler frequencies are not of interest, e.g., for spatial channel modeling. This paper proposes an improved hybrid sequential and random switching scheme. The primary purpose is to maintain the estimation accuracy of angles of MPCs while decreasing the resolution of Doppler frequencies for minimized complexity of channel parameter estimation. A simulated-annealing algorithm is exploited to obtain an optimized switching sequence. The effectiveness of the proposed scheme is also demonstrated with a realistic antenna array.

==> history.tex <==
%% Keep history

\section{hybrid switching and CRLB} \label{sec:3}
As mentioned in the introduction, a longer measurement time will lead to higher complexity in estimating the channel parameters. This is especially a problem when we do not aim for a high accuracy the Doppler estimation. One logical way to minimize this can be done by only taking a single channel measurement snapshot in situations where accurate the Doppler estimation is not the aim. However, when the sounding system has a massive number of antenna elements, even a single snapshot has a long measurement time, and a different approach must be considered. 


\begin{figure}[h]
    \centering
    \includegraphics[width=0.75\columnwidth]{images/Cylindrical_Sounder.jpg}
    \caption{\cite{bdb4a4ed338f46c8ae72fc4972961c13}, \cite{9329997}}
    % to do: delete last blue SS 
    \label{fig:sounder}
\end{figure}


\subsection{Hybrid Switching}
Assuming that the sounder is a cylindrical array, one way to reduce this effect can be done by dividing the antenna elements at the cylindrical array into different panels. Then we make sure that the switching order has a panel-wise uniform switching or as we call it, hybrid switching. In hybrid switching, the antenna switches through all possible antenna elements in the first panel then it switches through all antennas in the second panel and so on until the last panel. This means that hybrid sequences are the subset of switching sequences where the switching is uniform between panels but non-uniform within each panel. To find the optimal hybrid switching sequence, we use the exact same SA-based optimization algorithm presented in section II with a different $\textit{neighbor}(\boldsymbol{\eta})$ operation. Lets call the new neighbor picking operation for $\textit{neighbor}_{\textit{hybrid}}(\boldsymbol{\eta})$ and lets assume that we have $N_P$ panels then all what our $\textit{neighbor}_{\textit{hybrid}}(\boldsymbol{\eta})$ does is that in the first SA iteration, it swaps two rows in row $1$ to $N_P$ of $\eta$ then in the second SA iteration it swaps two rows in row $N_P+1$ to $2N_P$ and so on. Meaning that in each SA iteration we are picking the next panel and changing the switching order of two antenna elements in that panel.
 
 By doing this, we end up with an optimal hybrid switching sequence that gives us the extended Doppler range promised by Section II without the extra accuracy and complexity of the DF estimation. This is because a non-uniform switching sequence has a maximum switching time per panel equal to $M_R\cdot t0$ while a hybrid switching sequence reduces the maximum switching time per panel to $\frac{M_R\cdot t_0}{N_{P}}$.

Assuming that the sounder is a cylindrical array, one way to reduce this effect can be done by dividing the antenna elements at the cylindrical array into different panels. Then we make sure that the switching order has a panel-wise uniform switching or as we call it, hybrid switching. In hybrid switching, the antenna switches through all possible antenna elements in the first panel then it switches through all antennas in the second panel and so on until the last panel. This means that hybrid sequences are the subset of switching sequences where the switching is uniform between panels but non-uniform within each panel. To find the optimal hybrid switching sequence, we use the exact same SA-based optimization algorithm presented in section II with a different $\textit{neighbor}(\boldsymbol{\eta})$ operation. Lets call the new neighbor picking operation for $\textit{neighbor}_{\textit{hybrid}}(\boldsymbol{\eta})$ and lets assume that we have $N_P$ panels then all what our $\textit{neighbor}_{\textit{hybrid}}(\boldsymbol{\eta})$ does is that in the first SA iteration, it swaps two rows in row $1$ to $N_P$ of $\eta$ then in the second SA iteration it swaps two rows in row $N_P+1$ to $2N_P$ and so on. Meaning that in each SA iteration we are picking the next panel and changing the switching order of two antenna elements in that panel.
By doing this, we end up with an optimal hybrid switching sequence that gives us the extended Doppler range promised by Section II without the extra accuracy and complexity of the DF estimation. This is because a non-uniform switching sequence has a maximum switching time per panel equal to $M_R\cdot t0$ while a hybrid switching sequence reduces the maximum switching time per panel to $\frac{M_R\cdot t_0}{N_{P}}$.


\begin{dmath} \label{2}
    \mathbf{B}(\boldsymbol{\mu},
    \boldsymbol{\eta}_{\text{T}_{\text{H}}},
    \boldsymbol{\eta}_{\text{T}_{\text{V}}},
    \boldsymbol{\eta}_{\text{R}_{\text{H}}},
    \boldsymbol{\eta}_{\text{R}_{\text{V}}}) &=
        {\begin{bmatrix}
        (\bold{B}_{\text{T}_{\text{H}}} \odot \bold{A}_{\text{T}_{\text{H}}}) \diamond (\bold{B}_{\text{R}_{\text{H}}} \odot \bold{A}_{\text{R}_{\text{H}}}) \diamond \bold{B}_f \diamond \bold{B}_t \\
        (\bold{B}_{\text{T}_{\text{H}}} \odot \bold{A}_{\text{T}_{\text{H}}}) \diamond (\bold{B}_{\text{R}_{\text{V}}} \odot \bold{A}_{\text{R}_{\text{V}}}) \diamond \bold{B}_f \diamond \bold{B}_t \\
        (\bold{B}_{\text{T}_{\text{V}}} \odot \bold{A}_{\text{T}_{\text{V}}}) \diamond (\bold{B}_{\text{R}_{\text{H}}} \odot \bold{A}_{\text{R}_{\text{H}}}) \diamond \bold{B}_f \diamond \bold{B}_t \\
        (\bold{B}_{\text{T}_{\text{V}}} \odot \bold{A}_{\text{T}_{\text{V}}}) \diamond (\bold{B}_{\text{R}_{\text{V}}} \odot \bold{A}_{\text{R}_{\text{V}}}) \diamond \bold{B}_f \diamond \bold{B}_t \\
        \end{bmatrix}}^T 
\end{dmath}
where $\bold{B}_{\text{T}_{\text{H}}} \in \mathbb{C}^{M_{\text{T}} \times 1}$ and $\bold{B}_{{\text{T}_{\text{V}}}}\in \mathbb{C}^{M_{\text{T}} \times 1}$ represent the P path array responses at the Tx for the horizontal and the vertical polarizations. In the same manner,  $\bold{B}_{{\text{R}_{\text{H}}}}\in \mathbb{C}^{M_{\text{R}_{\text{H}}} \times P}$ and $\bold{B}_{{\text{R}_{\text{V}}}}\in \mathbb{C}^{M_{\text{R}_{\text{V}}} \times P}$ represent the Rx array responses. The matrix $\bold{B}_f\in \mathbb{C}^{M_f \times P}$ is the frequency basis matrix that depends on the time delay for the different paths and $\bold{B_t}\in \mathbb{C}^{M_t \times P}$ the response change due to the time between snapshots. Lastly, the matrices $\bold{A}_{T_{\text{T}_{\text{H}}}}\in \mathbb{C}^{M_{\text{T}_{\text{V}}} \times P}$, $\bold{A}_{\text{T}_{\text{V}}}\in \mathbb{C}^{M_{\text{T}_{\text{H}}} \times P}$, $\bold{A}_{\text{R}_{\text{H}}}\in \mathbb{C}^{M_{\text{R}_{\text{H}}} \times P}$  and $\bold{A}_{\text{R}_{\text{V}}}\in \mathbb{C}^{M_{\text{R}_{\text{V}}} \times P}$  represent the phase shifting caused by the switching sequences.

$\boldsymbol{\eta}_{\text{T}_{\text{H}}}\in \mathbb{R}^{M_{\text{T}_{\text{H}}} \times 1}$ and $\boldsymbol{\eta}_{\text{T}_{\text{V}}}\in \mathbb{R}^{M_{\text{T}_{\text{V}}} \times 1}$ represent the switching sequences of the horizontal polarized antennas and the vertical polarized antennas of Tx respectively. In the same fashion, $\boldsymbol{\eta}_{\text{R}_{\text{H}}}\in \mathbb{R}^{M_{\text{R}_{\text{H}}} \times 1}$ and $\boldsymbol{\eta}_{\text{R}_{\text{V}}}\in \mathbb{R}^{M_{\text{R}_{\text{V}}} \times 1}$ represent the switching timing at the Rx side. The elements in the phase weighting matrices are given by
\begin{equation}
  \begin{aligned}
        [\mathbf{A}_{\text{T}_{\text{H or V}}}]_{m_{\text{{T,p}}}} &= e^{j2\pi{\nu}_p[\boldsymbol{\eta}_{\text{T}_{\text{H or V}}}]_{m_{\text{T}}}}\\
        [\mathbf{A}_{\text{R}_{\text{H or V}}}]_{m_{\text{{R,p}}}} &= e^{j2\pi{\nu}_p[\boldsymbol{\eta}_{\text{R}_{\text{H or V}}}]_{m_{\text{R}}}}
   \end{aligned}
   \label{phase weighting vector}
\end{equation}
